Unified Path and Gait Planning for Safe Bipedal Robot Navigation

Safe path and gait planning are essential for bipedal robots to navigate complex real-world environments. The prevailing approaches often plan the path and gait separately in a hierarchical fashion, potentially resulting in unsafe movements due to neglecting the physical constraints of walking robots. A safety-critical path must not only avoid obstacles but also ensure that the robot's gaits are subject to its dynamic and kinematic constraints. This work presents a novel approach that unifies path planning and gait planning via a Model Predictive Control (MPC) using the Linear Inverted Pendulum (LIP) model representing bipedal locomotion. This approach considers environmental constraints, such as obstacles, and the robot's kinematics and dynamics constraints. By using discrete-time Control Barrier Functions for obstacle avoidance, our approach generates the next foot landing position, ensuring robust walking gaits and a safe navigation path within clustered environments. We validated our proposed approach in simulation using a Digit robot in 20 randomly created environments. The results demonstrate improved performance in terms of safety and robustness when compared to hierarchical path and gait planning frameworks.

==> sections/background.tex <==
% \section{Section}

% Section text here. 

% \subsection{Subsection Heading Here}
% Subsection text here.

% \subsubsection{Subsubsection Heading Here}
% Subsubsection text here.
\section{Method}

In this section, we first review the LIP model, a common bipedal model [], and present a corresponding LIP model-based MPC optimization problem to find the optimal controls for bipedal robots. Moreover, considering the safety factors, we also designed corresponding kinematic and environmental constraints based on the robot's walking characteristics. 
The goal is to provide a safe guaranteed obstacle avoidance path and generate corresponding controls for bipedal robots. 

\subsection{Linear Inverted Pendulum Model}
There are two expressions of the LIP model. One is the expression of the model in the local frame, which represents the CoM states of the robot in coordinates with the current stance foot as the origin []. In this expression, the coordinates need to be updated, and states also need to be transformed as the stance foot changes. The other expression is in the global frame, where both robot states and stance foot positions are expressed on a fixed coordinate system []. In our algorithm, we use the LIP model expressed in the global frame. This choice is because fixed coordinates can more easily represent obstacle information in the environment, such as CBFs. Moreover, using fixed coordinates prevents the robot's state from becoming discrete due to the frequent transformation needed to change coordinates.

\begin{figure}
\centering
\vspace{2mm}
    \begin{subfigure}[b]{0.48\linewidth}
         \centering
        \includegraphics[trim={7cm 0cm 8cm 0cm},clip,width=\linewidth]{Figures/LIP_ori.png}
         \caption{}
         \label{fig:LIP_ori}
     \end{subfigure}
     \begin{subfigure}[b]{0.47\linewidth}
         \centering
        \includegraphics[trim={8cm 0.5cm 7cm 0cm},clip,width=\linewidth]{Figures/LIP_dis_x.png}
         \caption{}
         \label{fig:LIP_x_dis}
     \end{subfigure}
     \begin{subfigure}[b]{1\columnwidth}
         \centering
        \includegraphics[trim={4cm 0cm 4cm 0cm},clip,width=\columnwidth]{Figures/LIP_new.png}
         \caption{}
         \label{fig:LIP_new}
     \end{subfigure}
\caption{\small{The Linear Inverted Pendulum Model. (a). The inverted pendulum locomotion in the x direction with a constant CoM height in the continuous time domain. (b). The inverted pendulum locomotion in the x direction with a fixed walking time duration. (c). The terminal states of the LIP model $\mathbf{x}_{k+1}$ switch its stance foot from $(f_{x_k}, f_{y_k})$ to $(f_{x_{k+1}}, f_{y_{k+1}})$ in the global frame}
} 
\vspace{-3.5mm}
\end{figure}

We use $H$ to denote the height of CoM of the robot and we assume the height of the robot would not change during the walking process. $g$ to denote the acceleration of gravity. Then the robot motion in the x-axis direction is:
\begin{align}
    \ddot{p_x} &= \frac{g}{H}(p_x-f_x)
\end{align}
where $p_x$ denotes the CoM position of the robot and $f_x$ denotes the stance foot displacement, see \figref{fig:LIP_ori}. We assume each walking step takes the same time duration $T$, and the robot is now at the beginning of time interval$[kT, (k+1)T)$. We define the initial position and velocity of the robot at the time $kT$ in the x-axis direction as $p_{x_k}$ and $v_{x_k}$, and the discrete foot displacement required at the current time is $f_{x_k}$, see \figref{fig:LIP_x_dis}. Then the closed-form solution of the robot terminal states at the end of the period is:
\begin{align}
\label{eq:x_dir_dynamics}
    \begin{bmatrix} p_{x_{k}+1} \\ v_{x_{k+1}} \end{bmatrix} =  \mathbf{A_d}
    \begin{bmatrix} p_{x_k} \\ v_{x_k} \end{bmatrix}
    + \mathbf{B_d}
    f_x
\end{align}
with: 
\begin{equation}
\label{eq:matrix_small}
\begin{aligned}
    \mathbf{A_d} &\coloneqq \left[ {\begin{array}{cc}
    \cosh(\beta t) & \frac{\sinh(\beta t)}{\beta}\\
   \beta\sinh(\beta t)  & \cosh(\beta t)
    \end{array} } \right]\\
    \mathbf{B_d} &\coloneqq \begin{bmatrix} 1-\cosh(\beta t) \\-\beta\sinh(\beta t) \end{bmatrix}
\end{aligned}
\end{equation}
where $\beta = \sqrt{g/H}$\\
For the 3D-LIP model, the motion in the y-axis direction is identical to the x-axis, and the turning of the heading is entirely independent of LIP control. Thus, we introduced an independent heading angle state $\theta$ and turning control $\phi$ to facilitate the subsequent construction of kinematic constraints.
The robot CoM states can be denoted as 
\begin{align}
\label{eq:states}
    \mathbf{x} \coloneqq [p_x, v_x, p_y, v_y, \theta]^T
\end{align}
and robot control:
\begin{align}
\label{eq:controls}
    \mathbf{u} \coloneqq [f_x, f_y, \phi]^T
\end{align}

Then, the modified 3D-LIP dynamics from step $k$ to step $k+1$ phase can be written as:

\begin{align}
\label{eq:system_dynamics}
    \mathbf{x}_{k+1} =  \mathbf{A}
    \mathbf{x}_k
    + \mathbf{B}\mathbf{u}_k
\end{align}
with: 
% \begin{equation}
% \label{eq:system_matrix}
% \begin{aligned}
%     \mathbf{A} &\coloneqq \begin{bmatrix}
%     \mathbf{A_d} & \mathbf{0}_{2\times2} & \mathbf{0}_{2\times1}\\
%     \mathbf{0}_{2\times2}& \mathbf{A_d} & \mathbf{0}_{2\times1}\\
%     \mathbf{0}_{1\times2} &  \mathbf{0}_{1\times2} & 1
%     \end{bmatrix} \\
%     \mathbf{B} &\coloneqq \begin{bmatrix} 
%     \mathbf{B_d} & \mathbf{0}_{2\times1} & \mathbf{0}_{2\times1}\\
%     \mathbf{0}_{2\times1} & \mathbf{B_d}  & \mathbf{0}_{2\times1}\\
%     0 & 0 & 1
%     \end{bmatrix}
% \end{aligned}
% \end{equation}
\begin{equation}
\label{eq:system_matrix}
\begin{aligned}
    \mathbf{A} &\coloneqq \begin{bmatrix}
    \mathbf{A_d} & \mathbf{0} & \mathbf{0}\\
    \mathbf{0}& \mathbf{A_d} & \mathbf{0}\\
    \mathbf{0} &  \mathbf{0} & 1
    \end{bmatrix} \\
    \mathbf{B} &\coloneqq \begin{bmatrix} 
    \mathbf{B_d} & \mathbf{0} & \mathbf{0}\\
    \mathbf{0} & \mathbf{B_d}  & \mathbf{0}\\
    0 & 0 & 1
    \end{bmatrix}
\end{aligned}
\end{equation}
where the dimension of matrix $A$ is $5\times5$, the dimension of matrix $B$ is $5\times3$.\\
Since the states and controls of the robot are defined in the global frame, the terminal states at the end of the previous time interval can be directly used as the initial states starting at the next time interval, see \figref{fig:LIP_new}, for example, $\mathbf{x}_{k+1}$ would be the initial states for time interval $[(k+1)T, (k+2)T)$.





\subsection{Discrete Control Barrier Function}
Consider robot discrete states $\mathbf{x}_k \in \mathcal{X}$ is the system state with $\mathcal{X}\subseteq \mathbb{R}^n$ being the state space, and $\mathbf{u}_k \in \mathcal{U}$ is the discrete control input with $\mathcal{U}\subseteq \mathbb{R}^m$ being the control space. If there exists a continuous and differentiable function $h: \mathbb{R}^n \rightarrow \mathbb{R}$, the safety set $\mathcal{C}$ of the system may be defined as []:
\begin{equation}
\label{eq:safety-set}
\begin{aligned}
    \mathcal{C} &= \{\mathbf{x}_k\in \mathbb{R}^n |h(\mathbf{x}_k) \geq 0\},\\
    \partial\mathcal{C} &= \{\mathbf{x}_k\in \mathbb{R}^n |h(\mathbf{x}_k) = 0\}.
\end{aligned}
\end{equation}
Then, $h$ is a control barrier function (CBF) if it follows the condition in the discrete-time domain for all $\mathbf{x}_k)\in\mathcal{C}$:
\begin{equation}
\label{eq:cbf_off}
\begin{aligned}
    \exists \text{ } \mathbf{u}_k &\text{ s.t. } \bigtriangleup h(\mathbf{x}_k, \mathbf{u}_k) \geq -\gamma(h(\mathbf{x}_k))
\end{aligned}
\end{equation}
where $\bigtriangleup h(\mathbf{x}_k, \mathbf{u}_k) \coloneqq h(\mathbf{x}_{k+1}) - h(\mathbf{x}_k)$, and $\gamma$ is a class $\kappa$ function that satisfies $0 < \gamma(h(x)) \leq h(x)$. In the discrete domain, $\gamma$ can be also a scalar that $0 < \gamma \leq 1$. So, the equation can be written as:
\begin{equation}
\label{eq:cbf_simp}
\begin{aligned}
    \exists \text{ } \mathbf{u}_k &\text{ s.t. } h(\mathbf{x}_{k+1}) + (\gamma - 1)h(\mathbf{x}_k) \geq 0
\end{aligned}
\end{equation}
Since the discrete control $\mathbf{u}_k$ is affine in (9 equ), it can be the DCBF constraint in MPC or QP to synthesize safe control.
